PageRank Bandits for Link Prediction

Link prediction is a critical problem in graph learning with broad applications such as recommender systems and knowledge graph completion. Numerous research efforts have been directed at solving this problem, including approaches based on similarity metrics and Graph Neural Networks (GNN). However, most existing solutions are still rooted in conventional supervised learning, which makes it challenging to adapt over time to changing customer interests and to address the inherent dilemma of exploitation versus exploration in link prediction. To tackle these challenges, this paper reformulates link prediction as a sequential decision-making process, where each link prediction interaction occurs sequentially. We propose a novel fusion algorithm, PRB (PageRank Bandits), which is the first to combine contextual bandits with PageRank for collaborative exploitation and exploration. We also introduce a new reward formulation and provide a theoretical performance guarantee for PRB. Finally, we extensively evaluate PRB in both online and offline settings, comparing it with bandit-based and graph-based methods. The empirical success of PRB demonstrates the value of the proposed fusion approach. Our code is released at https://github.com/jiaruzouu/PRB.

==> sources/tables/accuracy.tex <==
\begin{table*}[!t]
  \centering
  \caption{Average Accuracy of all methods on all datasets. \ban{To do: Transform regret to accuracy here.} }
  \vspace{-0.1em}
    % Table generated by Excel2LaTeX from sheet 'Sheet3'
    \scalebox{0.70}{
    \begin{tabular}{lcccccccc}
    \toprule
    \multirow{2}[4]{*}{Methods} &MovieLens & AmazonFashion& Facebook & GrQc & Pubmed & Citeseer & Cora \\
    \cmidrule{2-8} & Mean $\pm$ Std & Mean $\pm$ Std & Mean $\pm$ Std & Mean $\pm$ Std & Mean $\pm$ Std & Mean $\pm$ Std & Mean $\pm$ Std\\
    
     \midrule      
      PPR & & & & & & & \\
    EvePPR           & 9040 $\pm$ 17.2 & 4477 $\pm$ 14.4 & 9014 $\pm$ 17.9 & 9125 $\pm$ 17.9 & 8983 $\pm$ 16.8  & 8976 $\pm$ 21.9  & 9233 $\pm$ 15.2\\
    SEAL & & & & & & & \\
    NCNC & & & & & & & \\
    \midrule
    EE-Net           & \cellcolor[rgb]{ .776,  .937,  .808}1638 $\pm$ 15.3 & \cellcolor[rgb]{ .776,  .937,  .808} 1698 $\pm$ 19.3  & 2274 $\pm$ 27.1 & 3419 $\pm$ 16.5 & 1659 $\pm$ 11.3 & 2299 $\pm$ 33.4  & 1990 $\pm$ 13.8\\  
    NeuGreedy   & 1955 $\pm$ 17.3 & 1952 $\pm$ 27.4 & 2601 $\pm$ 14.2 & 3629 $\pm$ 18.2 & 1693 $\pm$ 13.5 & \jiaru{add later} & 2826 $\pm$ 21.4\\
    NeuralUCB        & 1737 $\pm$ 16.8 & 1913 $\pm$ 18.6 & 2190 $\pm$ 16.3 & 3719 $\pm$ 16.4 & 1672 $\pm$ 14.3 & 3101 $\pm$ 22.0  & 2713 $\pm$ 21.7\\
    NeuralTS         & 1683 $\pm$ 14.7 & 2055 $\pm$ 21.9 & 2251 $\pm$ 19.5 & 3814 $\pm$ 23.3 & 1647 $\pm$ 9.3 & 3419 $\pm$ 39.5  & 1998 $\pm$ 15.6\\
    \midrule
    PPB1             & 1892 $\pm$ 15.1 & 1741 $\pm$ 24.6 & \cellcolor[rgb]{ .776,  .937,  .808}1994 $\pm$ 23.6 & \cellcolor[rgb]{ .776,  .937,  .808}3332 $\pm$ 15.9 & 1634 $\pm$ 12.3  & 2194 $\pm$ 23.3  &1932 $\pm$ 24.1 \\
    PPB2             & \cellcolor[rgb]{ .776,  .937,  .808}1555 $\pm$ 21.7 & \cellcolor[rgb]{ .776,  .937,  .808}1617 $\pm$ 18.4 & \cellcolor[rgb]{ .776,  .937,  .808}1929 $\pm$ 17.0 & \cellcolor[rgb]{ .776,  .937,  .808}3236 $\pm$ 18.5 & 1577 $\pm$ 9.7  & 2168 $\pm$ 35.7 &1874 $\pm$ 25.6\\
    PPB2 (10\%-G)        & \cellcolor[rgb]{ .776,  .937,  .808}\textbf{1521 $\pm$ 17.6}  & \cellcolor[rgb]{ .776,  .937,  .808}\textbf{1565 $\pm$ 23.5} & \cellcolor[rgb]{ .776,  .937,  .808}\textbf{1858 $\pm$ 15.7} & \cellcolor[rgb]{ .776,  .937,  .808}\textbf{3085 $\pm$ 14.3} & - & - & -\\
    PPB2 (Full-G)  & - & - & - & - & 1630 $\pm$ 11.5  & 2158 $\pm$ 33.1  & 1804 $\pm$ 23.5\\

    \bottomrule
    \end{tabular}%
 }
  \label{tab:cell-selection}%
\end{table*}


==> sources/tables/rebuttal/bandit_inference.tex <==
\begin{table}[!ht]
    \caption{Inference Time (s) of PRB and bandit-based methods for each round}
    \centering
    \begin{tabular}{lccc}
    \toprule
        \textbf{Methods} & \textbf{MovieLens} & \textbf{GrQc} & \textbf{Amazon Fashion} \\ 
        \midrule
        NeuralUCB & 0.11 & 0.01 & 0.02 \\ 
        Neural Greedy & 0.14 & 0.02 & 0.03 \\ 
        EE-Net & 0.17 & 0.03 & 0.04 \\ 
        \midrule 
        \textbf{PRB} & 0.20 & 0.03 & 0.04 \\
        \bottomrule
    \end{tabular}   
\end{table}

==> sources/tables/rebuttal/graph_inference.tex <==
\begin{table}[!ht]
    \caption{Inference Time (s) of PRB and graph-based methods for the test set}
    \centering
    \begin{tabular}{lccc}
    \toprule
        \textbf{Methods} & \textbf{Cora} & \textbf{Pubmed} & \textbf{Collab} \\ 
        \midrule
        SEAL & 6.31 & 22.74 & 68.36 \\ 
        Neo-GNN & 0.12 & 0.24 & 9.47 \\ 
        Buddy & 0.27 & 0.33 & 2.75 \\ 
        NCNC & 0.04 & 0.07 & 1.58 \\ 
        \midrule
        \textbf{PRB} & 0.11 & 0.58 & 3.52 \\ 
        \bottomrule
    \end{tabular}
\end{table}

==> sources/tables/rebuttal/node_classification_acc.tex <==
\begin{table}[!ht]
\label{tab:rubuttal_node_classification_acc}
    \centering
    \caption{Offline Node Classification Accuracy}
    \begin{tabular}{lccc}
        \toprule
        \textbf{Methods} & \textbf{Cora} & \textbf{Citeseer} & \textbf{Pubmed} \\ 
        \midrule
        NueralTS & 73.2 & 66.5 & 82.4 \\
        NeuralUCB & 75.7 & 66.7 & 83.5 \\ 
        EE-Net & 77.1 & 70.8 & 84.2 \\ 
        \midrule
        \textbf{PRB} & 82.6 & 73.5 & 87.4 \\
        \bottomrule
    \end{tabular}
\end{table}
